Cryptographic Protocol for Multipart Missions Involving Two Independent and Distributed Decision Levels in a Military Context

In several critical military missions, more than one decision level are involved. These decision levels are often independent and distributed, and sensitive pieces of information making up the military mission must be kept hidden from one level to another even if all of the decision levels cooperate to accomplish the same task. Usually, a mission is negotiated through insecure networks such as the Internet using cryptographic protocols. In such protocols, few security properties have to be ensured. However, designing a secure cryptographic protocol that ensures several properties at once is a very challenging task. In this paper, we propose a new secure protocol for multipart military missions that involve two independent and distributed decision levels having different security levels. We show that it ensures the secrecy, authentication, and non-repudiation properties. In addition, we show that it resists against man-in-the-middle attacks.

==> rappel.tex <==
\section{Overview on increasing protocols}\label{sectionPreuveThFond}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       

Hereafter, we recall an important result: ''A protocol keeps its secret inputs when analyzed with a safe function and shown increasing''.

\subsection{Safe functions}
\begin{defini}{(Well-formed Function)}\label{bienforme}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. ${F}$ is ${\mathcal{C}}$-well-formed iff:
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}) \mbox{:}$\\

\begin{tabular}{rcl}
      $~~~{F}(\alpha,\{\alpha\})$ & $=$ & $\bot$ \\
   ${F}(\alpha,{M})~~~~$ & $=$ & $\top, \mbox{ if } \alpha \notin {\mathcal{A}}({M})$ \\   

      ${F}(\alpha, {M}_1 \cup {M}_2)$ & $=$ & ${F}(\alpha, {M}_1)\sqcap{F}(\alpha,{M}_2)$ \\
\end{tabular}
}$ $\\
\end{defini}

A well-formed function ${F}$ must return the infimum to a clear  atom $\alpha$ in $M$ to say that  anyone can know it if he knows $M$.  It returns the supremum to any atom $\alpha$ that does not appear in $M$ to say that nobody can know it if he knows  $M$. It  returns to an atom in the union of two sets, the minimum of the two values calculated in each set separately. This is to say that more the atom appears in messages more it is exposed to the intruder. \\

\begin{defini}{(Full-Invariant-by-Intruder Function)}\label{spi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification. 
${F}$ is full-invariant-by-intruder iff: $\forall {M} \subseteq {\mathcal{M}}, m\in {\mathcal{M}},  \alpha \in {\mathcal{A}}(m)$:\\
$
 {M} \models_{\mathcal{C}} m \Rightarrow ({F}(\alpha,m) \sqsupseteq{F}(\alpha,{M})) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner).
$\\
}
\end{defini}

A full-invariant-by-intruder function ${F}$ is such, when it affects a security level to an atom $\alpha$ in a set of messages $M$, the intruder cannot infer from this set a message $m$ in which this level decreases (i.e. ${F}(\alpha,m) \not \sqsupseteq{F}(\alpha,{M})$), unless he is explicitly authorized  to know it (i.e. $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$).\\

A function ${F}$ is s said to be safe if it is well-formed and full-invariant-by-intruder.\\



\begin{defini}{(${F}$-Increasing Protocol)}\label{ProAbsCroi}
{
Let ${F}$ be a function and ${\mathcal{C}}$ be a context of verification and $p$ be a protocol.\\
$p$ is ${F}$-increasing iff: $\forall R.r \in R_G(p), \sigma \in \Gamma,  \alpha \in {\mathcal{A}}(r^+), \mbox{ we have: }{F}(\alpha, r^+\sigma)\sqsupseteq \ulcorner \alpha \urcorner \sqcap{F}(\alpha, R^-\sigma)$
}
\end{defini}
$ $\\
An ${F}$-increasing protocol must produce traces with atomic messages having always a security level, returned by ${F}$, higher when sending (i.e. in $ r^+\sigma$) than when receiving (i.e. in $R^-\sigma$) or than its value in the context (i.e. $\ulcorner \alpha \urcorner$). \\


\begin{thm}{(Secrecy in Increasing Protocols)}\label{mainTh}
{
Let ${F}$ be a safe function and $p$ be an ${F}$-increasing protocol.
\begin{center}
$p$ keeps its secret inputs.
\end{center}
}
\end{thm}
$ $\\

Theorem \ref{mainTh} states that a protocol keeps its secret inputs when it is analyzed by a safe function $F$ and is shown increasing. This result is quite intuitive. In fact, if the intruder succeeds to obtain a secret $\alpha$ (clear) from the protocol then its security level given  by $F$ is the infimum since $F$ is well-formed. That cannot be due to the rules of the protocol  since this latter is $F\mbox{-increasing}$. That could not arise neither when the intruder uses his capabilities since $F$ is full-invariant-by-intruder. So, the secret is kept forever. The detailed proof is available in~\cite{Relaxed}.

\section{Guideline for Building Safe Functions}\label{sectionFonctionsetSelections}


In ~\cite{WitnessArt1} we propose a class  of safe selections: $S_{Gen}^{EK}$. Any selection $S$ in $S_{Gen}^{EK}$ must return to an atom $\alpha$ in a message $m$:

\begin{enumerate}
\item if $\alpha$ is encrypted by a key $k$ such that $k$ is the most external key that satisfies the condition $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ (we shortly call it the external protective key), a subset among $k^{-1}$ and the atoms that are neighbors of $\alpha$ under the same protection by $k$ ($\alpha$ itself is not selected);
\item for two messages joined by a function $f$ in $\Sigma$ other than an encryption by the protective key (e.g. pair), the union of two subselections in the two messages separately.
\item if $\alpha$ does not have a protective key in $m$, the infimum (all atoms);
\item if $\alpha$ does not appear in $m$, the supremum (the empty set);
\end{enumerate}

%%We prove that any $S\in S_{Gen}^{EK}$ is ${\mathcal{C}}$-safe.\\

Among the selections of $S_{Gen}^{EK}$, we point out three practical ones:
\begin{enumerate}
\item the selection $S_{MAX}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$, all the principal identities inside the same protection by $k$, in addition to $k^{-1}$;
\item the selection $S_{EK}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the external protective key $k$,  the key $k^{-1}$;
\item the selection $S_{N}^{EK}:$ it returns to an atom $\alpha$ in a message $m$ encrypted by the key external protective key $k$, all the principal identities inside the same protection by $k$;
\end{enumerate}
Any selection $S$ in $S_{Gen}^{EK}$ when composed to a suitable morphism $\psi$ returns a safe function $F=\psi \circ S$. 
We propose the morphism that returns for:
\begin{enumerate}
\item an agent, its identity;
\item the key $k^{-1}$, if selected, the set of agent identities  that know it.
\end{enumerate}
We denote by $F_{MAX}^{EK}, F_{EK}^{EK}$ and $F_{N}^{EK}$ respectively the functions resulting from the compositions $\psi \circ S_{MAX}^{EK}, \psi \circ S_{EK}^{EK}$ and $\psi \circ S_{N}^{EK}$. We prove~\cite{WitnessArt1} that these functions are safe. \\

\begin{comment}
The main idea of the proof is that the selection for any atoms (secrets) in any message takes place  in an invariant section protected by the key $k$. Therefore, to alter this section (to decrease the security level of an atom $\alpha$), the intruder must have previously obtained the atomic key $k^{-1}$. At this time, his knowledge must satisfy: $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner$. Since the key $ k^{-1}$ satisfies: $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ then the knowledge of the intruder must satisfy $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ as well since the operator "$\sqsupseteq$" is transitive. This is nothing but the definition of a full-invariant-by-intruder function. These functions are well-formed by construction, as well. Then, they are safe. 
\end{comment}


\begin{exemple}
Let us have the following context: $\ulcorner \alpha \urcorner=\{A, B, S\}$; $m=\{C.\{\alpha.D\}_{k_{as}}\}_{k_{ab}}$; ${k_{ab}^{-1}}={k_{ab}}, {k_{as}^{-1}}={k_{as}}$; $\ulcorner{k_{as}}\urcorner=\{A, S\}, \ulcorner{k_{ab}}\urcorner=\{A, B\}$. We have: \\
$S_{MAX}^{EK}(\alpha,m)=\{C, D, {k_{ab}^{-1}}\}$; \\
$F_{MAX}^{EK}(\alpha,m)=\psi\circ S_{MAX}^{EK}(\alpha,m)=\{C, D\}{ \cup}\ulcorner{k_{ab}^{-1}}\urcorner=\{C,D\} \cup \{A,B\}=\{A, B, C, D\}$.
\end{exemple} $ $\\

In all that follows, we refer to  any of the functions above by $F$ .

\section{Witness functions}\label{sectionWF}

The functions  we have  defined above can be used to analyze a protocol over its valid traces only. However, the set of valid traces is infinite. A static analysis could only be run over the finite set of generalized roles. Nevertheless, the messages in the generalized roles involve variables. We give here a safe way to use these functions in the presence of variables. For that, let us first instill the concept of derivation given by Definition \ref{derivation}.$ $\\ %% as shown in \ref{derivation}. 
$ $\\

\begin{defini}{[Derivation]}\label{derivation}
%%A derivative message is defined by the following rules:
%%\begin{table}[h]
%% \centering
\begin{center}
\begin{tabular}{rrcll}
~~~~~~& $\partial_X \alpha$ & $=$ & $\alpha$ &\\
& $\partial_X X$ & $=$& $\epsilon$ &\\
& $\partial_X Y~$ & $=$ & $Y, X\not = Y$ &\\
& $\partial{[\overline{X}]} m$ & $=$ & $\partial_{\{{\mathcal{X}}_m\backslash \{X\}\cup keys(m)\}} m$ &\\
& $\partial_X f(m)$ & $=$ & $ {f}(\partial_X m), f\in \Sigma$ &\\
& $\partial_{S_1 \cup S_2}m$ & $=$& $\partial_{S_1}\partial_{S_2}m$&\\ \\
\end{tabular}
\end{center}
%%\end{table}
\end{defini}

Derivation eliminates encrypted variables from a message. The expression $\partial m$ denotes $m$ where all encrypted variables inside are removed. Using derivation aims to get rid of variables that are neighbors of any analyzed atom by applying $F$ on the derivative message instead of the message itself. Any variable is evaluated as a block whatever its content (i.e quantified). A variable under evaluation (overlined) is not removed. This is described by Definition \ref{Fder}.
\begin{defini}\label{Fder}
$ $\\
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.\\
For all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, we denote by:
\[
F(\alpha, \partial [\overline{\alpha}] m\sigma) = \left\{
\begin{array}{ll}
F(\alpha,\partial m) & \mbox{if } \alpha \in {\mathcal{A}}(\partial m),\\
F(X,\partial [\overline{X}] m) & \mbox{if }\alpha \notin {\mathcal{A}}(\partial m) \\
%% & \mbox{and } \alpha \in {\mathcal{A}}(X\sigma). \\
& \mbox{and } \alpha =X\sigma. 
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma).\\
%% \underset{X \in {{\mathcal{X}}_m} } {\sqcap}

%% \mbox{ if } \alpha \not \in {\mathcal{A}}(\partial m) \mbox{ and }\alpha \in {\mathcal{A}}(X\sigma). \\
%% \\
%% \top & \mbox{ if } \alpha \not \in {\mathcal{A}}(m\sigma). \\

\end{array}
\right.
\]
\end{defini}

Although, the application given in Definition \ref{Fder} allows us to get rid of variables (neighbors), using it as it is to analyze protocols is not safe. Let us see the problem in Example \ref{exempleApp}.

\begin{exemple}\label{exempleApp}
Let $m_1$ and $m_2$ be two messages of a generalized role such that 
$m_1=\{\alpha.C.X\}_{k_{ab}}$ and $m_2=\{\alpha.Y.S\}_{k_{ab}}$ and $\ulcorner\alpha\urcorner=\{A,B,S\}$ and $\ulcorner{k_{ab}^{-1}}\urcorner=\{A,B\}$. Let $m=\{\alpha.C.S\}_{k_{ab}}$ be a valid trace. Let $F=F_{MAX}^{EK}$.\\
$$F(\alpha,\partial [\overline{\alpha}] m)=\begin{cases}
\{A, B, C\}&\!\!\!\!\! \mbox{if } m=m_1\sigma_1|X\sigma_1=S\\
\{A, B, S\}&\!\!\!\!\! \mbox{if } m=m_2\sigma_2|Y\sigma_2=C
\end{cases}$$
\end{exemple}

Thus, the application  in Definition \ref{Fder} is not necessarily a function since it may sometimes return more than one image for the same preimage. To fix this problem, we define the witness functions. A witness function  considers all the sources of the closed message $m\sigma$ (ground term) in the finite set  ${\mathcal{M}}_p^{\mathcal{G}}$, applies the application in Definition \ref{Fder} on all of them, and returns the minimum. This minimum must exist and is unique in a lattice. Since a secret is always evaluated under the protection of a protective key, the research  of the  sources of a closed message in ${\mathcal{M}}_p^{\mathcal{G}}$ is limited to the enryprtion patterns generated by the protocol. We denote by  $\tilde{\mathcal{M}}_p^{\mathcal{G}}$ the set of all these patterns.

\begin{defini}{[witness function]}\label{WF}
Let $m\in {\mathcal{M}}_p^{\mathcal{G}}$, $X \in {\mathcal{X}}_m$ and $m\sigma$ be a valid trace.
Let $p$ be a protocol and $F$ be a safe function. 
We define a witness function ${\mathcal{W}}_{p,F}$ for all $\alpha \in {\mathcal{A}}(m\sigma)$, $\sigma\in\Gamma$, as follows: 
%%On définit la fonction témoin sur les messages clos comme suit: 
\[{{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)=\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}} \otimes\Gamma.m'\sigma' = m \sigma \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F(\alpha, \partial [\overline{\alpha}] m'\sigma')\]
%%${\mathcal{W}}_{p,F}$ is said to be a witness function inside a protective key when $F$ is a verification Function such that its associated selection is an instance of the class $\Upsilon_{Gen}.$\\
\end{defini}

%%As we could see, a witness function depends on the set of sources of $m\sigma$ in ${\mathcal{M}}_p^{\mathcal{G}}$ (i.e. the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma.m'\sigma' = m \sigma\}$). So it depends on the substitution $\sigma$ that is not statically known. For that, we bind the witness function into two bounds that are independent of all substitution (runs). These bounds are provided by Proposition \ref{prePAT}.

Using a witness function as is to analyze a protocol is a very hard process since we cannot enumerate all the valid traces $m\sigma$ and their sources statically. For that we bind it into two bounds that do not depend on substitution (i.e on $\sigma$). The upper bound of a witness function returns a minimum set of confirmed principal identities for any $\alpha$ in $m$ whereas the lower bound returns the set of all principal identities from all the possible sources of $m$ (that are unifiable with it) including the odd ones.  The lower bound hunts so any odd principal identity and interprets it as an intrusion. The proof is quite simple since we have always  $\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}} \otimes\Gamma.m'\sigma' = m \sigma \} \subseteq \{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}} \otimes\Gamma.m'\sigma' = m \sigma' \}$ whatever $\sigma$. This is described by Proposition~\ref{prePAT}.

\begin{pre}{[binding a witness function]}\label{prePAT}
Let $m\in{\mathcal{M}}_p^{\mathcal{G}}$. Let ${\mathcal{W}}_{p,F}$ be a witness function.
For all $\sigma \in \Gamma$ we have:
$$F(\alpha,\partial[\overline{\alpha}] m)\sqsupseteq {{{\mathcal{W}}}}_{p,F}(\alpha,m\sigma)\sqsupseteq \!\!\!\! \!\!\!\! \!\!\! \underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}} \otimes\Gamma.m'\sigma' = m \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F(\alpha, \partial [\overline{\alpha}]m'\sigma')$$
\end{pre}



\section{Sufficient conditions for authentication}

Proposition \ref{PAT} states a decision criterion for secrecy  based on the bounds  of a witness function. The upper bound returns the set of the trusted identities only from the received message. The lower bound returns the set of all the identities including those that could be inserted by intruder by substituting a regular message when sent. The proof  of Proposition \ref{PAT} derives directly from Proposition \ref{prePAT} and Theorem \ref{mainTh}. \\

\begin{pre}{[Decision for Secrecy]}\label{PAT}
Let $p$ be a protocol. Let ${\mathcal{W}}_{p,F}$ be a witness function.
$p$ is correct with respect to secrecy if:
$\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$ we have:
$$\underset{{\{(m',\sigma') \in \tilde{\mathcal{M}}_p^{\mathcal{G}} \otimes\Gamma.m'\sigma' = r^+ \sigma' \}}}{\sqcap} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!F(\alpha, \partial[\overline{\alpha}] m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\partial[\overline{\alpha}] R^-)$$
\end{pre}

Theorem \ref{PAT2} sets two sufficient conditions for authentication. The first one makes sure that the protocol does not reveal its secrets. The second one makes sure that the link between a secret and the identity of the authenticatee is not broken.  For that, the upper bound of the witness function is called to confirm the presence of the authenticatee identity when the secret is evaluated in the  message that the authenticator receives from the authenticatee.\\

\begin{thm}{[Decision for Authentication]}\label{PAT2}
Let $p$ be a protocol. Let ${\mathcal{W}}_{p,F}$ be a witness function.
$p$ is correct with respect to authentication if:
\begin{enumerate}
\item Proposition \ref{PAT} holds;
\item Let $\alpha$ be the secret in a message $m$ received by an authenticator $B$ from an authenticatee $A$. We  have:
$$A \in F(\alpha, \partial[\overline{\alpha}] m) $$
\end{enumerate}
\end{thm}


It is easy to see that the conditions set by Theorem \ref{PAT2}  are statically checkable since they use the bounds of a witness function only, and both of them are statically calculable.
